Federated Multi-Task Learning under a Mixture of Distributions

The increasing size of data generated by smartphones and IoT devices motivated the development of Federated Learning (FL), a framework for on-device collaborative training of machine learning models. First efforts in FL focused on learning a single global model with good average performance across clients, but the global model may be arbitrarily bad for a given client, due to the inherent heterogeneity of local data distributions. Federated multi-task learning (MTL) approaches can learn personalized models by formulating an opportune penalized optimization problem. The penalization term can capture complex relations among personalized models, but eschews clear statistical assumptions about local data distributions. In this work, we propose to study federated MTL under the flexible assumption that each local data distribution is a mixture of unknown underlying distributions. This assumption encompasses most of the existing personalized FL approaches and leads to federated EM-like algorithms for both client-server and fully decentralized settings. Moreover, it provides a principled way to serve personalized models to clients not seen at training time. The algorithms' convergence is analyzed through a novel federated surrogate optimization framework, which can be of general interest. Experimental results on FL benchmarks show that our approach provides models with higher accuracy and fairness than state-of-the-art methods.

==> general_mtl_framework.tex <==
In this appendix, we give more details about the relation of our formulation with existing frameworks for (federated) MTL sketched in Section~\ref{sec:generalizing}. We suppose that Assumptions~\ref{assum:mixture}--\ref{assum:logloss} hold and that 
%Prop.~\ref{prop:local_model_is_weighted_average_of_components} enables us to have the first step in attributing the relation between Assum.~\ref{assum:mixture}, since other personalization approaches are interested in learning $h_{t}, t\in[T]$ directly. In the sequel, we consider that 
each client learns a predictor of the form~\eqref{eq:linear_combination}. Note that this is more general than  \cite{pmlr-v108-zantedeschi20a}, where each client learns a personal hypothesis as a weighted combination of a set of $M$ base \emph{known} hypothesis, since the base hypothesis and \emph{not only the weights} are learned in our case. 

\paragraph{Alternating Structure Optimization \cite{Zhou2011ClusteredMTLviaASO}.} Alternating structure optimization (ASO) is a popular MTL approach that learns a shared low-dimensional predictive structure on hypothesis spaces from multiple related tasks, i.e., all tasks are assumed to share a common feature space $P \in \mathbb{R}^{d' \times d}$, where $d' \leq \min(T, d)$ is the dimensionality of the shared feature space and $P$ has orthonormal columns ($PP^{\intercal}=I_{d'}$), i.e., $P$ is \emph{semi-orthogonal matrix}. ASO leads to the following formulation:
 \begin{equation}
        \label{eq:aso_formulation}
        \begin{aligned}
            \minimize_{W, P:PP^{\intercal}=I_{d'} } \quad & \sum_{t=1}^{T}\sum_{i=1}^{n_{t}}l\left(h_{w_{t}}\left(\vec{x}_{t}^{(i)}\right), y_{t}^{(i)}\right) + \alpha \left(\tr\left(W W ^{\intercal}\right) - \tr\left(WP^{\intercal}PW^{\intercal}\right)\right) + \beta \tr\left(W W ^{\intercal}\right),\\
        \end{aligned}
\end{equation}
where $\alpha \geq 0$ is the regularization parameter for task relatedness and $\beta \geq 0$ is an additional L2 regularization parameter. 

When the hypothesis $\left(h_{\theta}\right)_{\theta}$ are assumed to be linear, Eq.~\eqref{eq:linear_combination} can be written as $W = \Pi \Theta$. Writing the LQ decomposition\footnote{Note that when $\Theta$ is a full rank matrix, this decomposition is unique.} of matrix $\Theta$, i.e., $\Theta = LQ$, where $L \in \mathbb{R}^{M\times M}$ is a lower triangular matrix and $Q \in \mathbb{R}^{M  \times d}$ is a semi-orthogonal matrix ($Q Q^{\intercal} = I_{M}$), \eqref{eq:linear_combination} becomes $W = \Pi L Q \in \mathbb{R}^{T \times d}$, thus, $W = W Q^{\intercal} Q$, leading to the constraint $\left\|W - W Q^{\intercal} Q\right\|_{F}^{2} = \tr\left(W W ^{\intercal}\right) - \tr\left(WQ^{\intercal}QW^{\intercal}\right) = 0$. If we assume $\left\|\theta_{m}\right\|^{2}_{2}$ to be bounded by a constant $B>0$  for all $m \in[M]$, we get the constraint $\tr\left(W W^{\intercal} \right) \leq TB$. It means that minimizing $\sum_{t=1}^{T}\sum_{i=1}^{n_{t}}l\left(h_{w_{t}}\left(\vec{x}_{t}^{(i)}\right), y_{t}^{(i)}\right)$ under our Assumption~\ref{assum:mixture} can be formulated as the following constrained optimization problem
\begin{equation}
        \label{eq:constrained_pblm_aso}
        \begin{aligned}
            \minimize_{W, Q: QQ^{\intercal}=I_{M}} \quad & \sum_{t=1}^{T}\sum_{i=1}^{n_{t}}l\left(h_{w_{t}}\left(\vec{x}_{t}^{(i)}\right), y_{t}^{(i)}\right),\\
            \mathrm{subject \;\; to} \quad & \tr\left\{W W ^{\intercal}\right\} - \tr\left\{WQ^{\intercal}QW^{\intercal}\right\} = 0, \\
            & \tr\left(W W^{\intercal} \right) \leq TB.
        \end{aligned}
\end{equation}

Thus, there exists Lagrange multipliers $\alpha \in \mathbb{R}$ and $\beta > 0$, for which Problem~\eqref{eq:constrained_pblm_aso} is equivalent to the following regularized optimization problem
\begin{equation}
        \minimize_{W, Q:QQ^{\intercal}=I_{M} }  \sum_{t=1}^{T}\sum_{i=1}^{n_{t}}l\left(h_{w_{t}}\left(\vec{x}_{t}^{(i)}\right), y_{t}^{(i)}\right) + \alpha \left(\tr\left\{W W ^{\intercal}\right\} - \tr\left\{WQ^{\intercal}QW^{\intercal}\right\}\right) + \beta \tr\left\{W W ^{\intercal}\right\},
\end{equation}
which is exactly Problem~\eqref{eq:aso_formulation}. 

\paragraph{Federated MTL via task relationships.}
The ASO formulation above motivated the authors of~\cite{smith2017federated} to learn personalized models by solving the following problem
\begin{equation}
    \label{eq:virginia_app}
    \min_{W,\Omega} \sum_{t=1}^{T}\sum_{i=1}^{n_{t}}l\left(h_{w_{t}}\left(\vec{x}_{t}^{(i)}\right), y_{t}^{(i)}\right) +  \lambda \tr\left(W\Omega W^{\intercal}\right),
\end{equation}
Two alternative MTL formulations are presented in~\cite{smith2017federated} to justify Problem~\eqref{eq:virginia_app}: MTL with probabilistic priors~\cite{zhang2010convex} and  MTL with graphical models~\cite{lauritzen1996graphical}. Both of them can be covered using our Assumption~\ref{assum:mixture} as follows:
    \begin{itemize}
        \item Considering $T=M$ and $\Pi = I_{M}$ in Assumption~\ref{assum:mixture} and introducing a prior on $\Theta$ of the form 
            \begin{equation}
                \label{eq:prior_on_theta_app}
                \Theta \sim \left(\prod\mathcal{N}\left(0, \sigma^{2}I_{d}\right)\right) \mathcal{MN}\left(I_{d} \otimes \Omega \right)
            \end{equation}
        lead to a formulation similar to MTL with probabilistic priors \cite{zhang2010convex}.
        \item Two tasks $t$ and $t'$ are independent if $\langle \pi_{t}, \pi_{t'} \rangle  = 0$, thus using $\Omega_{t,t'} = \langle \pi_{t}, \pi_{t'} \rangle$ leads to the same graphical model as in \cite{lauritzen1996graphical}
    \end{itemize}
Several personalized FL formulations, e.g., \pFedMe \cite{dinh2020personalized}, \texttt{FedU} \cite{dinh2021fedu} and the formulation studied in \cite{hanzely2020federated} and in \cite{hanzely2020lower}, are special cases of formulation~\eqref{eq:prior_on_theta_app}.

